Efficient Iterative Processing in the SciDB Parallel Array Engine

Many scientific data-intensive applications perform iterative computations on array data. There exist multiple engines specialized for array processing. These engines efficiently support various types of operations, but none includes native support for iterative processing. In this paper, we develop a model for iterative array computations and a series of optimizations. We evaluate the benefits of an optimized, native support for iterative array processing on the SciDB engine and real workloads from the astronomy domain.

==> email.tex <==
Hello Magda, 

These are my thoughts about the sigmod paper. I would list the ideas then we can discuss tomorrow which one is more promising: 


1) Incremental optimization: This is basically what we have done so far. We define a wrapper around the regular arrays called "state array". Any array which is defined as a state array also keeps track of  \delta+ and \delta- values. We incrementally compute the result for aggregation functions sum(), count(), avg(), and stdv(). Each incremental function ƒ accompanied with a function ∂ which defines how to do ∂(ƒ(∆Ai), Ai) and generate pairs of (∆A_{i+1},A_{i+1}). So each incremental function is defined as a pair (ƒ,∂) and the only difference between a regular function and an incremental function is ∂. In our study we found that the body of the function ∂ is very similar for different functions ƒ in a sense that we always take item a_k from ƒ(∆Ai) and the corresponding item b_k from Ai, we apply scalar function c_k=s(a_k,b_k), if c_k is different than b_k then we update A_i, unless we let the b_k in Ai unchanged. So what we are basically passing to the system is (ƒ,s) instead of (ƒ,∂). 

For example for function ƒ equals to "sum" or "count" the "s" function is "sum" for \delta+ and "subtract" for \delta-. 
For example for function ƒ equals to "min" the "s" function is "min" for \delta+
 
summary: in each incremental function ƒ we also need to specify how to update the output state array.  


2) Hybrid of incremental and full computation: 
Functions ƒ such as min() and max() are not purely incremental operators because of the \delta- values ( because the minimum values could be in \delta- ) in this situation we do both incremental and full computation. Basically in each chunk c_i: 

1) we cache the sub-aggregate result of the previous iteration, name it Cache_i.
2) we compute incrementally ƒ(∆c_{i+1})=∆Cache_{i+1} and compare the result with Cache_i. Then we check the cells that the value ∆Cache_{i+1} is dominant compare to Cache_i. 
3) For those dominant cells we do full computation at c_i. 

Note that for (3), we first need to so some operation similar to extrusion filter in order to select those cells that contribute in the full computation. The performance gain is that hopefully only a small portion of cells contribute in the full computation phase.

For example: In the friends of friends use-case on the lsst dataset where we do slicing window with min() aggregation in each window, we first do the operation for \delta- values, then we check all the cells in the result that their corresponding ƒ(∆-)  is equal (dominant) to the current value of the result cell. Finally we do the full computation only for those cells. 

Summary: In this technique we are suggesting incremental operation + selective full computation. 

3) Overlap processing in iterative context: 

In the iterative overlap processing the challenge is that we need to update overlap cells at each chunk at each iteration. The way we propose to update the overlap cells is by a series of array operations as follow:

For iterative array A,

1) A_flat = unpack(A_overlap). which transform a multi-dimensional array into a result array with a single dimension, note we do unpack(...) only on A_overlap which are all the core cells in A that are contributing in the overlap cells.

2) redimension_store(A_flat,A), this has to update the overlap cells in array A. 

Note that redimension_store(..) involves network communication and is expensive. 

There are two ways to reduce the cost: 
1- The obvious optimization is to do unpacking on delta arrays to avoid sending core cells that has not changed. 
2- The second optimization is to run iterative computation ƒ multiple times locally in each chunk and then do one overlap-core cells synchronization. We can go further with this idea and reducing the cost by only participating those chunks in the synchronization that their total change in the A_overlap is more than a threshold T, here the meaning of "change" can be defined as a function like: total number of delta values in A_overlap or the total sum of delta values in A_overlap.

4) selective full computation for non-incremental operations.

    with the help of auxiliary statistics: 
    We restrict our binary operators to extrusion filter which is a special case for structural join. 
    ExtrusionFilter(A,B,ƒ(a,b)<=0) where A is the original array and B is the filter array. B slides through A       and at each step checks if the condition ƒ<=0 hold for corresponding cells "a" and "b". 

    The optimization is as follow: we initially compute and cache the result for min(A) and max(A).   
    for the next iterations, if ƒ(min(a),b) <=0 and ƒ(max(a),b)<=0 then we can exclude the cell b from the         computation. This optimization is valid as long as ƒ is a convex function. Note that in the extrusion             filter one cell in filter array B is compared with many cells in input array A, so this optimization saves a     lot of computation. 

    Example: extrusion filter in sigma-clipping use-case. 

   with the help of chunk re-organization and auxiliary statistics:  
   for non-incremental operators such as median(),K-rank(), and K-percentile(), we repartition each              chunk C into M inner chunks C_i such that for all the cells c \in C , m_i< val(c) < m_{i+1} are                        moved to C_i. The values in the set (m_1, ... , m_i, ... m_{M+1}) are determined by sampling over the        whole array. The auxiliary statistics that we use in this case is count() function. We compute the count()    for each of the C_i inner arrays. For the next iterations we use the count() value to skip those inner            chunks that do not have answer. Note that count() is an incremental function, so we can update our          count statistics incrementally in case changes (∆+,∆-) arrives. 

  For example in the case of 150-rank() and (m_1, .... ,m_11)=(0,10,...,100) and count(C_1) = 30
  count(C_2)=60 count(C_3)=40, and count(C_4)=40 ... 
  we can conclude that the result is in C_4, so we only compute the k-rank() for data that is in C_4. 
  
  I can assume the same scenario for the mode() function where we repartition each chunk to M inner  
  chunks based on the frequency of val(c) not its range.  









==> framework.tex <==
\section{Array Framework}
The array framework we propose is based on the work at~\cite{ewen:12}. The incremental iteration algorithm can be summarized as follow: 
\begin{algorithm}[ht] 
\scriptsize
\caption{Incremental iteration}
\label{alg:incr}
\begin{algorithmic}[1]
\STATE function INCR($\sigma,u,S,W$)
\WHILE{$W \ne \phi$}
\STATE $D \leftarrow u(S,W)$
\STATE $W \leftarrow \sigma(D,S,R)$
\STATE R some static data.
\STATE $S = S \cup D$
\ENDWHILE
\end{algorithmic}
\end{algorithm}


The $u$ and $\sigma$ functions because share a lot of states are sometimes combined and represented as one $\Delta$ function where $\{W_{i+1},S_{i+1}\} = \Delta(W_i,S_i)$
The difference in our framework and the work at~\cite{ewen:12} is the following:
\begin{enumerate}
\item In our framework the user defines state array $S$ and working set array $W$. Working set array could have the same schema as the state array (connected component example ) 
or it could have totally different schema ( $W$ is a 1d array centroids in kmeans while array $S$ is a multi-dimensional array representing points). 
\item $D_{i+1}$ is an array with the same schema as state array that represents the new states added or the existing states updated from the $u(S_i,W_i)$ computation. The difference of $D_i+1$ from the previous work at~\cite{ewen:12} is that this array could be a multi-versioned array . The user could define how to flatten array $D$ into one version array. The default action is the replacement with the latest version, but it could be merging all the versions of a particular cell with an aggregation function such as  $min()$,$count()$. The statement $S = S \cup D$ creates $S_{i+1}$. The $\cup$ function is by default the union function which picks values from $D$ if both corresponding cells are non-empty, but it could also be customized. 
\item $W$ is also a multi-version array. The way l look at it is as follow: Each new state-value $d$ in $D_i+1$ could send its value $d$ to other states either based on some static dependency pattern encoded as edges in the graph or some other functions. In other words each $d$ create one version of $W_i+1$. The user has the option the proactively combine/merge all the versions of $W_i+1$ before going to the next iteration or it could send $W_i+1$ with all of its versions to the function $u(S_i,W_i)$ for the next iteration. For example in the upcoming connected component example we could instead proactively call the $min()$ function on all the versions of $W_i+1$ in $\sigma(D_{i+1},S_i,E)$ function. 
\end{enumerate}
The following shows how the functions $u$ and $\sigma$ implemented in our framework for the connected component example:

\begin{verbatim}
\\sigma(D_i+1,S_i,E){
   W_i+1 = empty 
   TempArray = Project(Join(D_i+1,E, D_i+1.v_1 = E.v_1),label)
   for(k=0;k<TempArray.length;k++)
   	store(TempArray[k][*], W_i+1)
   return W_i+1
 }
\end{verbatim}

\begin{verbatim}
u(S_i,W_i){
   D_i+1 = empty  
   foreach( version W_ij in W_i)
   	D_i+1 = D_i+1 U Project(Filter(Join(W_ij,S, W_ij.v_1 = S.v_1),
         S.label > W_ij.label),W_ij.label)  
   return D_i+1
}
\end{verbatim}
The other idea that we had was about the granularity of states. In one hand we could have the finest granularity which makes the state and working set arrays large, and 
in the other hand we could have coarse grained states which incurs unnecessary communication overhead. We cannot makes state=chunks because chunks are the unit of 
I/O and are often selected very large size. Because versions are heavily involved in our array iterative framework, one idea is to choose \textit{virtual tiles} presented in our last paper as the same as the state size.  
%Now we describe how the connected component example fits into our \textit{iterative array processing framework}. The framework consists of the following 
%components. 
%\paragraph*{INIT()}
%At the \texttt{INIT} phase the user is required to define two arrays named \texttt{StateArray} and \texttt{WorkingArray}. 
%In this example both these arrays are equal and corresponds  to a 1D array with the following schema: \texttt{Array StateArray<int label>[v=0:n]} where each cell in the array corresponds to one node in the graph. Furthermore, the user optionally provides a static adjacency matrix $A$ which encodes the way $StateArray$ and $WorkingArray$ connected to each other. This is beneficial when the problem is inherently a graph problem where nodes only distribute new state values through their outgoing/incoming edges. The adjacency matrix for the graph $G$ in Figure~\ref{fig:cc-graph} is represented in Figure~\ref{fig:cc-adj-matrix}. At this phase both \texttt{StateArray} and the adjacency matrix  $A$ are partitioned across multiple machines. 
%\paragraph*{STtoWA()}
%This phase is intended to distribute new states calculated in the previous iteration to the relevant working array chunks. 
%In order to achieve that the user creates a \texttt{STtoWA} array. The user organizes and replicates the new state values in this array cells such that by partitioning the array, each working array chunk receives all the required new state values. For the connected component, the user specifies array \texttt{STtoWA} with the following schema: \texttt{Array STtoWA<int label>[v1=0:n,v2=0:n]} and then it filters out the cells that do not pass the the adjacency matrix $A$ followed by the join and project operation: \texttt{$\Pi$($\bowtie$($\sigma$(STtoWA, A) as F,StateArray as S, S.$v_1$=F.$v_1$),label)}. Figure~\ref{fig:cc-STtoWA} illustrates how to populate array \texttt{STtoWA} for the graph example $G$ in Figure~\ref{fig:cc-graph}. After array \texttt{STtoWA} is populated with the new state labels, it is re-shuffled column-based (illustrated in Figure~\ref{fig:cc-shuffle}).
%\paragraph*{COMPUTE()}
%This is the phase that we do the actual computation on the working arrays at each iteration. For the connected component example the working array and states are the same and corresponds to the label value in each vertex. Then the \texttt{COMPUTE} is simply calling $min$ aggregation function on the new states received from the previous step and update the label value on your vertex based on the following formula: $l_i = min(l_i, \min_{\{v_i,v_j\} \in E} l_j)$. Notice in general at the end of the computation phase the algorithm might generate new state values that is not local to the working array chunk (\eg Transitive Closure Algorithm). So we need an optional state reshuffling step at the end of each \texttt{COMPUTE} phase if necessary. 
%\paragraph*{TERMINATION\_CHECK()}
%Each time after the \texttt{COMPUTE} phase, the \texttt{TERMINATION\_CHECK} is triggered. This phase could be either a UDF function written by the user to check for the end of iteration, or simply a counter which increases each time the \texttt{TERMINATION\_CHECK()} function is called, or in case none of them is provided the system by default checks  whether new state values generated at the end of \texttt{COMPUTE} phase. 
%\begin{figure*}[t]
%\begin{center}
%\subfigure[Adjacency matrix for the graph $G$]{
%\includegraphics[width=0.3\linewidth]{img/cc-adj-matrix.pdf}
%\label{fig:cc-adj-matrix}
%}
%\subfigure[Each state $S_i$ corresponding to node $V_i$ populates its new value to all the states $S_j$ where $\{v_i,v_j\} \in E$. The results are 
%stored in a array called \texttt{STtoWA} ]{
%\includegraphics[width=0.3\linewidth]{img/cc-STtoWA.pdf}
%\label{fig:cc-STtoWA}
%}
%\subfigure[\texttt{STtoWA} array is partitioned column-based. After shuffling is finished, each node in the graph receives labels from its neighbors (It is highlighted for node $V_5$)
%. Then It picks the minimum label which in arrays corresponds to \texttt{min} aggregate function on array \texttt{STtoWA} group by column. ]{
%\includegraphics[width=0.32\linewidth]{img/cc-shuffle.pdf}
%\label{fig:cc-shuffle}
%}
%\caption{}
%\label{}
%\end{center}
%\end{figure*}


==> header.tex <==
% ***********************************************************
% ******************* PHYSICS HEADER ************************
% ***********************************************************
% Version 2
%\documentclass[11pt]{article} 
\usepackage{amsmath} % AMS Math Package
\usepackage{amsthm} % Theorem Formatting
\usepackage{amssymb}	% Math symbols such as \mathbb
\usepackage{graphicx} % Allows for eps images
\usepackage{multicol} % Allows for multiple columns
\usepackage[dvips,letterpaper,margin=0.75in,bottom=0.5in]{geometry}
 % Sets margins and page size
\pagestyle{empty} % Removes page numbers
\makeatletter % Need for anything that contains an @ command 
\renewcommand{\maketitle} % Redefine maketitle to conserve space
{ \begingroup \vskip 10pt \begin{center} \large {\bf \@title}
	\vskip 10pt \large \@author \hskip 20pt \@date \end{center}
  \vskip 10pt \endgroup \setcounter{footnote}{0} }
\makeatother % End of region containing @ commands
\renewcommand{\labelenumi}{(\alph{enumi})} % Use letters for enumerate
% \DeclareMathOperator{\Sample}{Sample}
\let\vaccent=\v % rename builtin command \v{} to \vaccent{}
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} % for vectors
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
% for vectors of Greek letters
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} % for unit vector
\newcommand{\abs}[1]{\left| #1 \right|} % for absolute value
\newcommand{\avg}[1]{\left< #1 \right>} % for average
\let\underdot=\d % rename builtin command \d{} to \underdot{}
\renewcommand{\d}[2]{\frac{d #1}{d #2}} % for derivatives
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} % for double derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} 
% for partial derivatives
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} 
% for double partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
 \right)_{#3}} % for thermodynamic partial derivatives
\newcommand{\ket}[1]{\left| #1 \right>} % for Dirac bras
\newcommand{\bra}[1]{\left< #1 \right|} % for Dirac kets
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
 \left. #2 \vphantom{#1} \right>} % for Dirac brackets
\newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
 #2 \left| #3 \vphantom{#1#2} \right>} % for Dirac matrix elements
\newcommand{\grad}[1]{\gv{\nabla} #1} % for gradient
\let\divsymb=\div % rename builtin command \div to \divsymb
\renewcommand{\div}[1]{\gv{\nabla} \cdot #1} % for divergence
\newcommand{\curl}[1]{\gv{\nabla} \times #1} % for curl
\let\baraccent=\= % rename builtin command \= to \baraccent
\renewcommand{\=}[1]{\stackrel{#1}{=}} % for putting numbers above =
\newtheorem{prop}{Proposition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\theoremstyle{definition}
\newtheorem{dfn}{Definition}
\theoremstyle{remark}
\newtheorem*{rmk}{Remark}

% ***********************************************************
% ********************** END HEADER *************************
% ***********************************************************

